Language Model Adaptation to Specialized Domains through Selective Masking based on Genre and Topical Characteristics

Recent advances in pre-trained language modeling have facilitated significant progress across various natural language processing (NLP) tasks. Word masking during model training constitutes a pivotal component of language modeling in architectures like BERT. However, the prevalent method of word masking relies on random selection, potentially disregarding domain-specific linguistic attributes. In this article, we introduce an innovative masking approach leveraging genre and topicality information to tailor language models to specialized domains. Our method incorporates a ranking process that prioritizes words based on their significance, subsequently guiding the masking procedure. Experiments conducted using continual pre-training within the legal domain have underscored the efficacy of our approach on the LegalGLUE benchmark in the English language. Pre-trained language models and code are freely available for use.

==> tables/results_LAMA.tex <==
\begin{table*}[htbp]
\centering

\label{tab:legallama_res}
\resizebox{\textwidth}{!}{% Resize table to fit the page width
\begin{tabular}{l *{10}{S[table-format=2.1]}}
\toprule
\textbf{Task} & \multicolumn{3}{c}{\textbf{Statistics}} & \multicolumn{7}{c}{\textbf{Models}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-11} &
%{\#T} & {\#L} & {\#T/\#L} &
{B} & {LB} & {LB-CFT} & {LB-RW} & {LB-T\_N} & {B-CFT} & {MB-T\_N} & {MB-RW} & {MB-TFIDF} \\
\midrule
ECHR Articles     %& 69 & 13 & 1.0 &
38.42 & 91.11 & 91.20 & 91.91 & 92.17 & 42.80 & 72.81 & 67.57 & 45.51\\
Contract Sections %& 85 & 20 & 1.3 &
35.38 & 80.21 & 79.23 & 75.05 & 74.89 & 42.24 & 22.09 & 22.20 & 39.24\\
Contract Types    %& 150 & 15 & 1.1 &
46.63 & 82.22 & 78.85 & 76.14 & 77.21 & 44.11 & 38.10 & 39.23 & 42.46\\
Crime Charges (US)%& 118 & 59 & 2.1 &
38.82 & 51.46 & 50.03 & 37.03 & 38.28 & 42.17 & 5.49 & 22.16 & 43.34\\
Terminology (US)  %& 92 & 7 & 2.9 &
36.97 & 60.55 & 60.15 & 40.08 & 40.37 & 45.36 & 17.91 & 18.94 & 47.71\\
Terminology (EU)  %& 164 & 42 & 3.0 &
37.45 & 63.18 & 64.94 & 50.66 & 47.24 & 49.58 & 30.06 & 32.71 & 53.19\\
Terminology (CoE) %& 97 & 250 & 1.2 &
35.55 & 77.26 & 79.39 & 58.88 & 57.49 & 57.38 & 24.24 & 27.25 & 57.35\\
CC Sections       %& 72 & 144 & 2.0 &
8.07 & 21.86 & 23.33 & 7.96 & 6.58 & 18.83 & 5.49 & 6.32 & 11.80 \\
\bottomrule
\end{tabular}
}
\caption{The 8 LegalLAMA tasks’ statistics regarding the average number of tokens in the input (\#T), the number of labels to predict from (\#L), and the average number of tokens per label (\#T/L) along with the Mean Reciprocal Rank results of all examined PLMs.}
\end{table*}

==> test.tex <==
Récemment Frantzi & Ananiadou [1996] et Nakagawa [2001] ont pris conscience de la nécessité
d’appréhender davantage les cas d’imbrication d’expressions (respectivement avec la C-value et l’Imp).
C’est pourquoi nous étudierons leur application pour notre problème d’extraction de méta-descripteurs,
bien que ces mesures restent toujours très sensibles à la définition d’un seuil optimal de sélection.x

a l'instar de X et Y qui ont proposé des mesures de la spécificité au domaine nous proposer un score pour mesurer la scpécificité au genre BIBER. Notre travail s'inspire 
